Transferable Latent-to-Latent Locomotion Policy for Efficient and Versatile Motion Control of Diverse Legged Robots

Reinforcement learning (RL) has demonstrated remarkable capability in acquiring robot skills, but learning each new skill still requires substantial data collection for training. The pretrain-and-finetune paradigm offers a promising approach for efficiently adapting to new robot entities and tasks. Inspired by the idea that acquired knowledge can accelerate learning new tasks with the same robot and help a new robot master a trained task, we propose a latent training framework where a transferable latent-to-latent locomotion policy is pretrained alongside diverse task-specific observation encoders and action decoders. This policy in latent space processes encoded latent observations to generate latent actions to be decoded, with the potential to learn general abstract motion skills. To retain essential information for decision-making and control, we introduce a diffusion recovery module that minimizes information reconstruction loss during pretrain stage. During fine-tune stage, the pretrained latent-to-latent locomotion policy remains fixed, while only the lightweight task-specific encoder and decoder are optimized for efficient adaptation. Our method allows a robot to leverage its own prior experience across different tasks as well as the experience of other morphologically diverse robots to accelerate adaptation. We validate our approach through extensive simulations and real-world experiments, demonstrating that the pretrained latent-to-latent locomotion policy effectively generalizes to new robot entities and tasks with improved efficiency.

==> rlw.tex <==
\section{Related Works}

\subsection{Latent Space Representations in Robotic Locomotion}

Latent space representations offer a compact, high-level abstraction of complex sensorimotor data, enabling robots to learn and execute locomotion tasks more efficiently. Mitchell et al. (2020) introduced a framework where a deep generative model captures feasible joint configurations in a latent space, allowing for the optimization of locomotion trajectories under complex constraints. This approach demonstrated that latent space control could be successfully applied to real-world quadruped robots, such as the ANYmal platform. \cite{mitchell2020latent}

Similarly, Li et al. (2020) proposed a hierarchical framework that jointly learns a low-level controller and a high-level latent action space. This method enables planning over continuous latent actions using a learned high-level dynamics model, facilitating generalization to multiple robots, including hexapods and quadrupeds. \cite{li2020planning}

\subsection{Transfer Learning in Legged Robot Locomotion}

Transfer learning has been instrumental in enhancing the adaptability of locomotion controllers across different robots and environments. Jiang et al. (2020) introduced an evolutionary gait transfer framework that utilizes pre-acquired knowledge to accelerate gait optimization in complex terrains. By applying transfer learning, their approach demonstrated improved efficiency in adapting to various terrains compared to non-transferred scenarios. \cite{jiang2020evolutionary}

Furthermore, Smith et al. (2023) developed a framework for training complex robotic skills by transferring experience from existing controllers. This method enables robots to learn agile behaviors, such as jumping and navigating on hind legs, by leveraging prior knowledge, thereby reducing the need for extensive retraining. \cite{smith2023transfer}

\subsection{Integration of Latent Space and Transfer Learning}

The combination of latent space representations and transfer learning has led to more robust and adaptable locomotion controllers. Rezaei-Shoshtari et al. (2021) explored the use of latent space to capture a lower-dimensional representation of complex dynamics in robotic systems. Their work demonstrated that latent space representations could effectively model and infer interactions in tasks such as cutting, highlighting the potential for these methods in various robotic applications. \cite{rezaei2021heterogeneous}

These advancements underscore the potential of combining latent space representations with transfer learning to develop locomotion controllers that are both efficient and adaptable, paving the way for more versatile legged robots capable of operating in diverse environments.


==> table/rec_loss_tab.tex <==
% \aboverulesep = 1mm
% \belowrulesep = 1.4mm

\begin{table}[t]
\centering
\caption{Accuracy and Reward Performance benchmark}
\label{tab.sim_result}

\newcommand{\Aa}{10.11\%   &   15.77\%   &   9.97\%   &   \cellcolor{lightgray!10}{\textbf{7.14\%}}}
\newcommand{\Ab}{0.52\%   &   1.17\%   &   0.57\%   &   \cellcolor{lightgray!10}{\textbf{0.35\%}}}
\newcommand{\Ac}{2.73\%   &   4.43\%   &   4.85\%   &   \cellcolor{lightgray!10}{\textbf{2.63\%}}}
\newcommand{\Ba}{0.25\%   &   0.47\%   &   0.32\%   &   \cellcolor{lightgray!10}{\textbf{0.20\%}}}
\newcommand{\Cc}{363.99   &   345.44   &   371.41   &   \cellcolor{lightgray!10}{\textbf{374.48}}}

\begin{threeparttable}
\begin{tabular}{lllccccc}
\toprule

{Metrics} &\multicolumn{3}{c}{Average curriculum on playground}&\multicolumn{1}{c}{\cellcolor{lightgray!10}{Final}}\\

\cmidrule(lr){2-4} \cmidrule(lr){5-5} & Boxes & Up-Stairs & Down-Stairs & \cellcolor{lightgray!10}{Average} \\
             
\midrule
Original        $\downarrow$        & \Aa \\
Recover         $\downarrow$        & \Ab \\
Nearest center  $\downarrow$        & \Ac \\

\midrule

Acc  AED $\downarrow$      & \Ba \\
\midrule
TAR $\uparrow$        & \Cc \\

\bottomrule

\end{tabular}

\vspace{3pt}
\begin{tablenotes}\footnotesize
\item[*] For MED and AED, we use $\downarrow$ to denote lower value means better.
\item[*] For TAR, we use $\uparrow$ to denote higher value means better.
\item[*] Bold indicates the best.
\end{tablenotes}

\end{threeparttable}

\end{table}
